Semidefinite relaxations for certifying robustness to adversarial examples

Despite their impressive performance on diverse tasks, neural networks fail catastrophically in the presence of adversarial inputs---imperceptibly but adversarially perturbed versions of natural inputs. We have witnessed an arms race between defenders who attempt to train robust networks and attackers who try to construct adversarial examples. One promise of ending the arms race is developing certified defenses, ones which are provably robust against all attackers in some family. These certified defenses are based on convex relaxations which construct an upper bound on the worst case loss over all attackers in the family. Previous relaxations are loose on networks that are not trained against the respective relaxation. In this paper, we propose a new semidefinite relaxation for certifying robustness that applies to arbitrary ReLU networks. We show that our proposed relaxation is tighter than previous relaxations and produces meaningful robustness guarantees on three different "foreign networks" whose training objectives are agnostic to our proposed relaxation.

==> fig-tighten.tex <==
\begin{figure}
  \centering
  \includegraphics[scale = 0.4 ]{layerwise_one}
  \caption{The relation between the linear and quadratic versions of the
    output of the ReLU units that are infered by the simple SDP are not
    the tightest possible. If we had an estimate of $l$ and $u$,
  we can add the tight linear constraint to get a new tighter SDP}
\end{figure} 


==> figs-lp.tex <==
\begin{figure}
\centering 
\begin{subfigure}[t]{0.4\textwidth}
  \centering
  \includegraphics[scale = 0.25]{figs/one_reluD}
  \caption{}
  \label{fig:lp-1}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
  \centering
  \includegraphics[scale = 0.05]{figs/lp-2}
  \caption{}
  \label{fig:lp-2}
\end{subfigure}
\caption{a) Illustration of $\sZ^{\text{LP}}$ and $\sZ^\text{SDP}$ for a single ReLU unit
  b) At the optimal configuration for the simple construction, the
  input $\vec{x}$ is the sum of $d$ orthogonal vectors. It can be easily seen that $\| \vec{z} \| \leq \| \vec{x}\|$
and hence $\vec{z} \cdot \unit =O(\sqrt{d} \epsilon)$.}
\end{figure}


==> figs-one.tex <==
\begin{figure}
%% \centering
%% \begin{subfigure}[t]{0.49\textwidth}
%% \centering
%% \includegraphics[scale=0.35]{one-relu}
%% \caption{}
%%   \label{fig:one-relu}
%% \end{subfigure}
%% \phantom{xx}
%% \begin{subfigure}[t]{0.45\textwidth}
%% \centering
%% \includegraphics[scale=0.25]{tight-relu}
%% \caption{}
%%   \label{fig:tight-relu}
%% \end{subfigure}
\centering 
\begin{subfigure}[t]{0.3\textwidth}
  \centering
  \includegraphics[scale = 0.2]{figs/one_reluA}
  \caption{$l < 0 < u$}
\end{subfigure}
\begin{subfigure}[t]{0.3\textwidth}
  \centering
  \includegraphics[scale = 0.2]{figs/one_reluB}
  \caption{$l, u >0$}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
  \centering
  \includegraphics[scale = 0.2]{figs/one_reluC}
  \caption{$l, u < 0$}
\end{subfigure}
\caption{Illustration of the convex set $\sZ^{\text{SDP}}$,
when $\sX = \{ x \mid x^2 \leq (l + u) - lu \}$ for different values of $l$ and $u$. \js{isn't the shape of the relaxation also a function of how big $l$ and $u$ are relative to each other, not just the sign of $l$ and $u$?}}
\label{fig:one}
\end{figure}

